CVA6-VMRT: A Modular Approach Towards Time-Predictable Virtual Memory in a 64-bit Application Class RISC-V Processor

The increasing complexity of autonomous systems has driven a shift to integrated heterogeneous SoCs with real-time and safety demands. Ensuring deterministic WCETs and low-latency for critical tasks requires minimizing interference on shared resources like virtual memory. Existing techniques, such as software coloring and memory replication, introduce significant area and performance overhead, especially with virtualized memory where address translation adds latency uncertainty. To address these limitations, we propose CVA6-VMRT, an extension of the open-source RISC-V CVA6 core, adding hardware support for predictability in virtual memory access with minimal area overhead. CVA6-VMRT features dynamically partitioned Translation Look-aside Buffers (TLBs) and hybrid L1 cache/scratchpad memory (SPM) functionality. It allows fine-grained per-thread control of resources, enabling the operating system to manage TLB replacements, including static overwrites, to ensure single-cycle address translation for critical memory regions. Additionally, CVA6-VMRT enables runtime partitioning of data and instruction caches into cache and SPM sections, providing low and predictable access times for critical data without impacting other accesses. In a virtualized setting, CVA6-VMRT enhances execution time determinism for critical guests by 94% during interference from non-critical guests, with minimal impact on their average absolute execution time compared to isolated execution of the critical guests only. This interference-aware behaviour is achieved with just a 4% area overhead and no timing penalty compared to the baseline CVA6 core.

==> tab/std_dev_result_tab.tex <==
\begin{table}[t]
    \begin{center}
    \setlength{\tabcolsep}{1.5pt} % Tune column width
    \renewcommand{\arraystretch}{1.3} % Tune row height (vertical spacing)
    \begin{tabular}{lrr}

    \toprule

    \multirow{2}{*}{\rotatebox{0}{\textbf{Mitigations}}} &
    \multirow{2}{*}{\rotatebox{0}{\textbf{\makecell[cc]{Synthetic \\ Benchmark}}}} & 
    \multirow{2}{*}{\rotatebox{0}{\textbf{\makecell[cc]{Powerwindow \\ Benchmark}}}}\\
    \\
    \midrule

    \textbf{None} & 71 & 15793\\
    \textbf{\gls{tlb} part. \& locking + SPM} & 6 & 953\\
    \midrule
    \textbf{Improvement} & 91\% & 94\%\\

    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Execution time standard deviation (in clock cycles) for both benchmarks in the unmitigated and fully mitigated cases.}
    \label{tab:improvement}
    \end{center}
\end{table}
